Randomized and Deterministic Maximin-share Approximations for Fractionally Subadditive Valuations

We consider the problem of guaranteeing maximin-share (MMS) when allocating a set of indivisible items to a set of agents with fractionally subadditive (XOS) valuations. For XOS valuations, it has been previously shown that for some instances no allocation can guarantee a fraction better than $1/2$ of maximin-share to all the agents. Also, a deterministic allocation exists that guarantees $0.219225$ of the maximin-share of each agent. Our results involve both deterministic and randomized allocations. On the deterministic side, we improve the best approximation guarantee for fractionally subadditive valuations to $3/13 = 0.230769$. We develop new ideas on allocating large items in our allocation algorithm which might be of independent interest. Furthermore, we investigate randomized algorithms and the Best-of-both-worlds fairness guarantees. We propose a randomized allocation that is $1/4$-MMS ex-ante and $1/8$-MMS ex-post for XOS valuations. Moreover, we prove an upper bound of $3/4$ on the ex-ante guarantee for this class of valuations.

==> src/exantepost.tex <==
\section{Ex-ante and Ex-post Guarantees} 

Unfortunately, the randomized allocation obtained by Theorem \ref{thm:1} has no ex-post fairness guarantee. The issue is that we use  Theorem \ref{thm:fei} to convert the fractional allocation into a randomized one. However, Theorem \ref{thm:fei} only guarantees that the ex-post value of each agent is at least the value of her fractional allocation minus the value of the heaviest item which is partially (and not fully) allocated to her in the fractional allocation. However, currently, we have no upper bound on the value of the allocated items, and therefore, the ex-post value of an agent might be close to $0$. To resolve this, we perform two improvements on our allocation. 

First, we allocate valuable items beforehand to keep the value of the remaining items as small as possible. 
We start by using a simple and very practical fact that is frequently used in previous studies~\cite{ghodsi2018fair,seddighin2022improved,barman2017approximation,amanatidis2019multiple}: allocating one item to one agent and removing them from the instance does not decrease the maximin-share value of the remaining agents for the remaining items. 

\begin{lemma}\label{ass:1}
	Removing one item and one agent from the instance does not decrease the maximin-share value of the remaining agents for the remaining items.
\end{lemma}

Given that our goal is to construct a randomized allocation which is $1/4$-$\MMS$ ex-ante, by Lemma \ref{ass:1} we can assume without loss of generality that the value of each item to each agent is less than $1/4$; otherwise, we can reduce the problem using Lemma \ref{ass:1}.
However, a combination of this assumption and Theorem \ref{thm:1} still gives no ex-post guarantee: the ex-ante guarantee obtained by Theorem \ref{thm:1} is $1/4$-$\MMS$ and assuming that the value of each item to each agent is less than $1/4$ implies no lower-bound better than $0$ on the ex-post $\MMS$ guarantee. 
To improve the ex-post guarantee, we revisit the proof of Theorem \ref{thm:fei} and show that for our setting, a stronger guarantee can be achieved using the matching method for converting a fractional allocation into a randomized one. Indeed, we show that we can find a fractional allocation with a special structure that makes the transformation step more efficient. These ideas together help us achieve a randomized allocation with $1/4$-$\MMS$ guarantee ex-ante and $1/8$-$\MMS$ guarantee ex-post.

\ExAnteExPost*
%\begin{theorem}\label{thm:2}
%	There exists a randomized allocation that is $1/4$-$\MMS$ ex-ante and $1/8$-$\MMS$ ex-post.
%\end{theorem}
In the rest of this section, we prove Theorem \ref{thm:2}. The algorithm we use for proving Theorem \ref{thm:2} is as follows:
\begin{enumerate}
	\item While there exists a remaining item with a value of at least $1/4$ to a remaining agent, satisfy her with that item and remove them from the instance. 
	\item Start with an arbitrary integral allocation and consider $\bar{\valu}_i$ as defined in Equation \eqref{vbar} as the valuation function of agent $i$. While it is possible, improve the allocation (using the method we describe later).
	\item Convert the final fractional allocation into a randomized allocation using Lemma \ref{lem:fractorand}.
\end{enumerate}

%\todo{Label the steps and reference them.}
Recall that by Lemma \ref{ass:1}, we know that after the first step, the maximin-share value of the remaining agents for remaining items is at least $1$. For simplicity, we scale the valuations after the first step and assume that the $\MMS$ value of each remaining agent after the first step is exactly equal to $1$. Also, we suppose that the number of agents that are satisfied in the first step is $n_1$. Therefore, $n-n_1$ agents head to the second step. %\HA{We can just say that any solution satisfying the remaining agents can be extended to a solution satisfying all the agents simply by allocating the goods that are allocated in the first step to the corresponding agents. This way, we reduce the instance to one that no item is of value at least $1/4$ to any agent. So without loss of generality, we can assume we have $n$ agents, for all agents $i$ and item $b_j$, $\MMS_i=1$ and $v_i(\{b_j\})<1/4$. No need to have $n_1$.}


%Given Claim \ref{cl:1} and Observation \ref{obs:4}, 
The goal in Step (ii) is to find a fractional allocation that is $1/4$-$\MMS$. However, we want this allocation to have a special structure that facilitates constructing the randomized allocation.  Therefore, instead of directly choosing the allocation that maximizes social welfare, we proceed as follows: Consider $\bar{\valu}_i$ as the valuation function of agent $i$ and start with an arbitrary integral allocation $\falloc$. If in $\falloc$, all the agents have a value of at least $1/4$ for their bundles, then we are done. Otherwise, we choose one of the agents, namely agent $i$, that has a value less than $1/4$ for her share. By Claim \ref{clm:divide}, we know that agent $i$ can distribute all the items (items that have remained after the first step) into $2(n-n_1)$ bundles each with value at least $1/2$ to her. Here, we construct these $2(n-n_1)$ bundles more carefully.
% Recall the way we construct these bundles in Claim \ref{cl:1}: each one of these $2(n-n_1-n_2)$ bundles is obtained from a bundle in one of sets  $B_0, B_1,$ and $B_2$. The bundle we extract from each bundle in $B_1 \cup B_2$ is integral, that is, no item is fractionally present in these bundles.

Indeed, for every bundle in the optimal partitioning of agent $i$, we construct two bundles with a value of at least $1/2$ as follows: we divide each item into two half-unit items and put each half-unit into one bundle. That way, we can say that in each one of these $2(n-n_1)$ bundles, each item is either integrally present in one bundle \HA{How can an item be integrally present in one bundle? Only the following case can arise.}, or there are two bundles each of which contains one half of that item. More formally, for every agent $i$ and item $\ite_j$, we have $f_{i,j} \in \{0,1/2,1\}$.  

Using the same deduction as we used in the proof of Theorem \ref{thm:2}, we can say that since the number of remaining agents after the first step is $n-n_1$, the value of one agent for her bundle is less than $1/4$, and value of the rest of the agents for their bundles is at most $1/2$, the social welfare of the allocation is less than $(n-n_1)/2$. Therefore, at least one of these $2(n-n_1)$ bundles, say $B_k$ contributes less than $1/4$ to social welfare. Now we take back these items from other agents and allocate them to agent $i$. The reallocation increases social welfare as shown in the proof\footnote{Let $\falloc'$ be the allocation (see Program~\ref{eq:contr}) that defines the contribution of bundle $B_k$ to allocation $\falloc$.  Then $\sum_i f'_{ij} = \sum_i f_{ij} - b_{kj}$ for all $j$ and
{$\sum_{1 \leq i \leq n} \bar{\valu}_i(\falloc) -  \sum_{1 \leq i \leq n} \bar{\valu}_i(\falloc') =  C_{\bar{v}}^\falloc(B_k) <1/4$}. We now assign the items in $B_k$ to agent $i$, i.e., we consider the fractional allocation $\falloc''$ equal to $\falloc'$, except that for agent $i$, we have 
	$$
	\forall_{1 \leq j \leq m} \qquad f''_{i,j} = f'_{i,j} + b_{k,j}.
	$$
        Since the value of bundle $B_k$ to agent $a$ is at least $1/2$, we have {$\bar{\valu}_{i}(\falloc'') - \bar{\valu}_{i}(\falloc') >1/4$}, and hence 
$\sum_{1 \leq i \leq n} \bar{\valu}_i(\falloc'') >  \sum_{1 \leq i \leq n} \bar{\valu}_i(\falloc)$. The change from $\falloc$ to $\falloc'$ takes back the fractional items in $B_k$ from the other agents and the change from $\falloc'$ to $\falloc''$ allocates them to agent $i$.} of Theorem \ref{thm:1}. \label{footnote}

Note that this process eventually terminates, since at each step the social welfare increases. When the process terminates, we know that for the final allocation $\falloc$, we have that for every agent $i$, $\valu_i(\falloc) \geq 1/4$. Also, for every agent $i$ and item $\ite_j$, we have $f_{i,j} \in \{0,1/2,1\}$. Therefore, the following Observation holds.

\begin{observation}\label{obs:stupper}
	Let $\falloc$ be the allocation after Step (ii). Then, for every agent $i$ we have $\valu_i(\falloc) \geq 1/4$. Furthermore, for every item $\ite_j$, we have $f_{i,j} \in \{0,1/2,1\}$. 
\end{observation}

Now, we show how to convert $\falloc$ into a randomized allocation. Recall that the result of Theorem \ref{thm:fei} does not provide us with an ex-post guarantee better than $0$.  
Here, we give a more accurate analysis to prove that the outcome of our algorithm is $1/8$-$\MMS$.  Our construction is based on the Birkhoff---von Neumann theorem: Every fractional perfect matching can be written as a linear combination of integral perfect matchings. We adopt the construction to our setting and, in particular, exploit the fact that all $f_{ij}$ are half-integral.

%{\color{blue} In this section, we prove Lemma~\ref{lem:2}. In \cite{babaioff2022best} it was shown how to convert a randomized allocation into a probability distribution over integral allocations. The construction is based on the Birkhoff---von Neumann theorem: Every fractional perfect matching can be written as a linear combination of integral perfect matchings. We adopt the construction to our setting and, in particular, exploit the fact that all $f_{ij}$ are half-integral.
	
	\begin{lemma} \label{lem:fractorand} Assume that the valuations are additive and let $\falloc$ be a complete fractional allocation with $f_{ij} \in \{0, 1/2, 1\}$ for all $i$ and $j$. Then there is a randomized allocation $\ralloc$ with $\domain(\ralloc) = \{\allocation^1,\allocation^2\}$, such that
		\begin{itemize}
			\item  For every agent $i$ we have $\valu_i(\ralloc) = \valu_{i}(\falloc)$. 
			%\item If $f_{ij} = 1$, $\ite_j$ is allocated to $i$ in both allocations, if $f_{ij} = 1/2$, $\ite_j$ is allocated to $i$ in one allocation, but not the other, and if $f_{ij} = 0$, $\ite_j$ is not allocated to $i$ in either allocation.
			\item For every agent $i$ we have  
			\[ \min\bigg\{\valu_{i}(\allocation^1_i),\valu_{i}(\allocation^2_i)\bigg\}\geq  v_i(\ralloc) - \frac{\max \{ v_i(b_j)\, | \, f_{ij} = 1/2\}}{2}. \]
		\end{itemize}
	\end{lemma}
	\begin{proof}
		For each agent $i$, let $f_i = \sum_j f_{ij}$.  Since $\sum_i f_i= m$,  the number of agents with non-integral $f_i$ is even. We pair the agents with non-integral $f_i$ arbitrarily. For each pair, we create a new dummy item with a value of zero for all the agents and assign one-half of the dummy item to each agent in the pair. In this way, for every agent $i,$  $f_i$ becomes an integer. Therefore, for the rest of the proof we assume that for every agent $i$, $f_i$ is an integer.
		
		We now construct allocations $\allocation^1$ and $\allocation^2$ such that $f_{ij}$ is equal to the fraction of allocations in $\ralloc$ that allocate item $\ite_j$ to $i$, i.e., if $f_{ij} = 1$ we allocate $\ite_j$ to $i$ in both allocations, if $f_{ij} = 0$, we allocate $\ite_j$ to $i$ in neither allocations, and if $f_{ij} = 1/2$ we allocate $\ite_j$ to $i$ in exactly one of the two allocations. For brevity, we define $\items_{1/2}$ and $\agents_{1/2}$ as follows:
		\begin{align*}
			\items_{1/2} &= \{\ite_j| \exists i: f_{i,j} = 1/2\}\\
			\agents_{1/2} &= \{i| \exists \ite_j: f_{i,j} = 1/2 \}
		\end{align*}
		
		Consider a bipartite graph $G(X,Y)$ with parts $X$ and $Y$ as follows: For every item $\ite_j \in \items_{1/2}$  there is a vertex $y_j$ in $Y$ corresponding to item $\ite_j$. For every agent $i \in \agents_{1/2}$, we have vertices $x^1_i,x^2_i,\ldots,x_i^{t_i}$ in $X$, where $t_i$ is half the number of items $\ite_j$ such that $f_{ij} = 1/2$, that is
		$$
		t_i = \frac{\big|\{\ite_j| f_{i,j} = 1/2\}\big|}{2}.
		$$
		Also, we add the following edges to $G$. For every $i \in \agents_{1/2}$, order the items $\ite_j$ with $f_{ij} = 1/2$ in decreasing order of their value to agent $i$. Then we connect $x_i^1$ to the first two items, $x^2_i$ to the items with ranks three and four, and so on. In this way, all vertices in $X$ and $Y$ have degree two. 
		Hence, $G$ decomposes into vertex disjoint cycles. Each cycle decomposes into two matchings (note that since the graph is bipartite, all the cycles have even length), and thus $G$ decomposes into two perfect matchings, say $M^1$ and $M^2$. We define allocations $\allocation^1$ and $\allocation^2$ as follows: for every item $\ite_j$, agent $i$, and $r \in \{1,2\}$, we allocate item $\ite_j$ to agent $i$ in $\allocation^r$, if and only if either $f_{i,j} = 1$, or $M^r(y_j) = x_i^k$ for some $1 \leq k \leq t_i$, where $M^r(y_j)$ refers to the vertex matched with $y_j$ in $M^r$. Define $\ralloc$ as a randomized allocation that selects $\allocation^1$ or $\allocation^2$, each with probability $1/2$. 
		
		It is easy to check that for every agent $i$, $\valu_{i}(\ralloc) = \valu_{i}(\falloc)$. Here, we focus on the ex-post guarantee of $\ralloc$. Fix an agent $i$ and Let $b_1$, $b_2$, \ldots, $b_{2t_i}$ be the items half-owned by $i$ in order of decreasing value for agent $i$. Then, by the way we construct $M^1$ and $M^2 $, for all $1 \le \ell \le t_i$, $b_{2\ell - 1}$ and $b_{2\ell}$ are allocated to $i$ in different allocations. Hence, the value of the $i^{\textrm{th}}$ bundle in either allocation $\allocation^r$ satisfies
		\[    v_i(\allocation_i^r) \ge v_i(b_2) + v_i(b_4) + \ldots + v_i(b_{2t_i}) + \sum_{j: f_{i,j}=1} \valu_i(\{\ite_j\}) .\]
		We can now bound $v_i(\falloc) - v_i(\allocation_i^r)$ from above. %The $j$ with $f_{ij} \in \{0,1\}$ cancel out. 
		%For the $j$ with $f_{ij} = 1/2$ we obtain
		\begin{align*}
			v_i(\falloc) - v_i(\allocation_i^r) &\le \frac{1}{2} \left(\sum_{1 \le \ell \le 2t_i} v_i(b_\ell) \right)  -  \sum_{1 \le \ell \le t_i} v_i(b_{2\ell}) \\
			&= \frac{v_i(b_1)}{2} + \sum_{1 \le \ell < t_i} \left(\frac{v_i(b_{2\ell}) + v_i(b_{2\ell+1})}{2} - v_i(b_{2\ell})\right) + \frac{v_i(b_{2t_i})}{2} - v_i(b_{2t_i})\\
			&\le  \frac{v_i(b_1)}{2}.
		\end{align*}
	\end{proof}
	
	Finally, let $\allocation^1$ and $\allocation^2$ be the integral allocations obtained by Lemma \ref{lem:fractorand}. Consider any agent $i$, and let $u_{i,i'}$ be such that $v_i(\ralloc) = \sum_j f_{ij} u_{i,i'}(b_j)$. Then, by Lemma \ref{lem:fractorand} for $r \in \{1,2\}$ we have
	\[  u_{i,i'}(\allocation_i^r) \ge u_{i,i'}(\ralloc_i^\ell) - \frac{\max \{u_{i,i'}(b_j) \, \vert\, f_{i,j} = 1/2\}}{2}\]
	and since by Lemma \ref{ass:1} we know the value of each item for each agent is less than $1/4$, we have 
	\[ v_i(\allocation_i^\ell) \ge v_i(\ralloc_i) - \frac{\max_j v_i(b_j)}{2} > \frac{1}{4} - \frac{1}{8} = \frac{1}{8}.\]
	
%\input{src/extra.tex}	


==> src/expost.tex <==
\section{Ex-post Guarantee}\label{sec:expost}
In this section, our goal is to improve the best approximation guarantee of $\MMS$ for deterministic allocations in the fractionally subadditive setting. Here, we show that guaranteeing a factor $0.22962$ of maximin-share to all the agents is always possible. Before this work, the best approximation guarantee for maximin-share in the $\XOS$ setting was $0.219225$\GS{$0.2173913$}-$\MMS$~\cite{seddighin2022improved}.

Our algorithm for improving the ex-post guarantee is based upon \HA{on} our previous algorithms plus an additional step and a more  in-depth analysis. In this algorithm, before finding the allocation that maximizes social welfare, we strengthen our upper bound on the value of items. For this, we add another step to our algorithm that satisfies some of the agents with two items. In contrast to the first step \HA{(i.e., allocating single items to agents)}, this step might decrease the maximin-share value of the remaining agents for the remaining items. 
Let $t \leq 1/2$ be a threshold that we fix later and assume that the goal is to find a $t/2$-$\MMS$ allocation. Our allocation algorithm is as follows:
\begin{enumerate}
	\item If there exists an item $\ite_{j}$ with value at least $t/2$ to an agent $i$, allocate $\ite_j$ to agent $i$ and remove $i$ and $\ite_j$ respectively from the items and the agents. \KM{Reassign the other items in the bundle containing $\ite_j$ arbitrarily}. \HA{We do not need to actually reassign the other items in the bundle. This is only an argument to show the $\MMS$ value of a remaining agent does not drop but not part of our algorithm.}
	\item If there exists a pair of items $\ite_{j},\ite_k$ with the total value of at least $t/2$ to some agent $i$, allocate $\ite_{j},\ite_k$ to agent $i$ and remove them from the items and remove agent $i$ from the agents. \KM{If $\ite_j$ and $\ite_k$ belong to the same bundle, reassign the other items in the bundle arbitrarily. If they belong to different bundles, merge the two bundles into one.}
	\item For the remaining agents and items, proceed as follows: for every agent $i$, define $\bar{\valu}_i$ as follows: 
	$$\forall S \subseteq \items \quad \bar{\valu}_i(S) = \min(t,\valu_{i}(S)).$$
	Consider $\bar{\valu}_i$ as the valuation function of agent $i$ and return an (integral) allocation that maximizes social welfare.
\end{enumerate}

In the rest of this section, we analyze the above algorithm.
First, by Lemma \ref{ass:1} we can suppose that after the first step, the maximin-share value of each remaining agent for the remaining items is equal to $1$. Also, after the first step, the value of each item to each agent is less than $t/2$. We denote by $n_1$, the number of agents that are satisfied in the first step. 

\begin{observation}\label{obs:4}
	Since no item can satisfy any remaining agent, after Step (i), for every agent $i$ and every item $\ite_j$, we have 
	$\valu_{i}(\{\ite_j \})<t/2	$. 
\end{observation}

In the second step, we satisfy some of the agents with two items. In contrast to the first step, this step might decrease the maximin-share value of the remaining agents for the remaining items. However, we prove that the remaining items satisfy special structural property. We denote by $n_2$, the number of agents that are satisfied during the second step.
We prove that after the second step, Claim \ref{cl:1} holds. 

\begin{claim}\label{cl:1}
	Fix a remaining agent $i$ and consider the $n-n_1$ bundles with value at least $1$ in the optimal $\MMS$-partitioning of agent $i$ after the second step. %we know agent $i$ has $n-n_1$ bundles with value at least $1$ in her optimal $\MMS$-partition. We 
	Put these bundles into  5 \HA{3} different sets $B_0, B_1, B_2, B_3, B_{\geq 4}$ \HA{$B_{\geq 2	}$}, where for $0 \leq \ell \leq 3$, set $B_\ell$ contains bundles that lose exactly $\ell$ items in the second step, and $B_{\geq4}$ contains bundles that lose more than 4 items in the second step. 
After Step $(ii)$, the following inequality holds:
	$$
2(n-n_1-n_2) \leq 2B_0 + B_1 + B_2.
	$$
 \GS{$2|B_0| + |B_1| + |B_2|$}
	\HA{$$
		2(n-n_1-n_2) \leq 2B_0 + B_1.
		$$
        In particular, if $B_0 = 0$, then $2(n - n_1 - n_2) \le B_1$. }

\end{claim}
\begin{proof}
	Since each satisfied agent in the second step receives two items, $2n_2$ items are allocated to the satisfied agents in this step. Given the definition of $B_0,B_1,B_2,B_3,B_{\geq 4}$, we have:
	\begin{equation}\label{ineq:1}
			2n_2 \geq {|B_1| + 2|B_2|+3|B_3|+4|B_{\geq 4}|}.
		\end{equation}
	%We show that $2|B_0| + |B_1| + |B_2| \geq 2(n-n_1-n_2)$.  
        Note that  we have 
	\begin{equation}\label{ineq:2}
			|B_0| + |B_1| + |B_2| + |B_3| + |B_{\geq 4}| = n-n_1.
		\end{equation}
	Now, using Inequality \eqref{ineq:1} we have
	\begin{align}
			2(n-n_1)-2n_2 &\leq 2(n-n_1)-|B_1| -2|B_2| - 3|B_3| - 4|B_{\geq 4}| \nonumber\\
			&\leq 2B_0 + B_1 -B_3 - 2B_{\geq 4}&\mbox{ Inequality \eqref{ineq:2}}\nonumber\\
			&\leq 2B_0 + B_1 + B_2. \text{ \HA{We can remove $B_2$.}}\label{inq:upper}
		\end{align}
\end{proof}

Also, since after Step $(ii)$, no pair of items can satisfy an agent, after this step the following observation holds.
\begin{observation}\label{obs:5}
	After Step $(ii)$, for every items $\ite_j,\ite_k$ and every agent $i$ we have $\valu_{i}(\{\ite_j,\ite_k\}) < t/2$.
\end{observation}
Note that since the valuations are $\XOS$, Observation \ref{obs:5} implies no upper bound better than $t/2$ on the value of a single item to an agent. For example, consider the following extreme scenario: for a small constant $\epsilon>0$, the value of every subset of items to agent $i$ is equal to $t/2-\epsilon$. It is easy to check that this valuation function is $\XOS$. For this case, the value of every pair of items is also equal to $t/2-\epsilon$, but this implies no upper bound  better than $t/2$ on the value of a single item.



Finally, in the third step, we find the integral allocation $\allocation$ that maximizes social welfare with respect to $\bar{\valu}_i$ for agent $i$. Let 
$$
Z = \sum_i \bar{\valu}_i(\allocation_i).
$$

Since the number of remaining agents in Step $(iii)$ is $n-n_1-n_2$, and for each remaining agent $i$, $\KMtwo{\valu}{\bar{\valu}}_{i}(\allocation_i)$ is upper-bounded by $t$, we have $Z \KMtwo{<}{\le} (n-n_1-n_2)t$. If for every agent $i$, $\valu_{i}(\allocation_i)\geq t/2$ holds, then $\allocation$ is $t/2$-$\MMS$, and we are done. Therefore, suppose that for an agent $i$, we have $\valu_{i}(\allocation_i)<t/2$.

Recall the definition of sets $B_0,B_1,$ and $B_2$ for agent $i$ from Claim \ref{cl:1}. Since each bundle of $B_1 \cup B_2$ loses at most 2 items in the second step, by Observation \ref{obs:4}, the total value of the remaining items in each bundle in $B_1 \cup B_2$ is at least $1/2>t$.
Hence, given that $\allocation$ maximizes social welfare, the contribution of each of these extracted bundles to $Z$ is more than $t/2$; otherwise, we can increase social welfare by taking back the items in that bundle from the rest of the agents and giving them to agent $i$. \KM{The argument is as in the proof of Theorem~\ref{1/4 ex-ante} and the footnote on page~\pageref{footnote}}. Therefore, we have
$$
\sum_{B \in B_1 \cup B_2} C_{\allocation}(B) > (|B_1|+|B_2|)t/2. 
$$
Thus,
by Lemma \ref{lem:supper-additive}, we have
\begin{align*}
\sum_{B \in B_0} C_{\allocation}(B) &< Z-(|B_1|+|B_2|)t/2\\
&<(n-n_1-n_2)t - (|B_1| + |B_2|)t/2.
\end{align*}
%
% in $B_0$ to $Z$ is less than $$Z' = (n-n_1-n_2)t - (|B_1|+|B_2|)t/2.$$
Hence, the contribution of at least one of the bundles that are in $B_0$ is less than
\begin{align}
	\frac{(n-n_1-n_2)t - (|B_1|+|B_2|)t/2}{|B_0|}
	&\KMtwo{=}{\le} \frac{(2|B_0| +|B_1| + |B_2|)t/2 - (|B_1|+|B_2|)t/2}{|B_0|} \nonumber&\mbox{By Inequality \eqref{inq:upper}}\\
	&=\frac{|B_0|t}{|B_0|} \nonumber\\
	&=t \label{ineq:contr}.
\end{align} \KM{\textbf{What if $|B_0| = 0$?} It is conceivable that all bundles are in $B_1$. Say $n_2 = (n - n_1)/2$ and $2n_2 = 2 | B_1|$. } \HA{Then, since the contribution of each bundle in $B_1$ is at least $t/2$, $Z=tn_2$ and thus every agent is receiving a bundle of value $t/2$.}
We denote such a bundle by $B$. To summarize, bundle $B$ satisfies the following properties:
\begin{itemize}
	\item $\mathsf{(C_1)}$: Since $B \in B_0$, value of $B$ to agent $i$ is at least 1.
	\item $\mathsf{(C_2)}$: By Inequality \eqref{ineq:contr}, the contribution of $B$ to $Z$ is less than $t$. 
	\item $\mathsf{(C_3)}$: By Observation \ref{obs:5}, value of every pair of items in $B$ to agent $i$ is less than $t/2$.
	\item $\mathsf{(C_4)}$: By maximality of $Z$, we know that for every subset $S \subseteq B$, taking the items in $S$ back from their owners in $\allocation$ and allocating them to agent $i$ does not increase social welfare, i.e.,
	\begin{equation}\label{eq:cont}
		\forall_{S \subseteq B}\qquad \big(\bar{\valu}_i\left(S \cup \allocation_i\right)- \bar{\valu}_i\left(\allocation_i\right)\big) - C_\allocation(S) \leq 0.
	\end{equation}
	Note that
	\begin{align*}
		\big(\bar{\valu}_i\left(S \cup \allocation_i\right)- \bar{\valu}_i\left(\allocation_i\right)\big) - C_\allocation(S) &= \min(t, \valu_i(S \cup \allocation_i) ) - \bar{\valu}_i(\allocation_i) -  C_\allocation(S) \\
		&>  \min(t, \valu_i(S \cup \allocation_i) ) - t/2 - C_\allocation(S).
	\end{align*}  
\end{itemize} 

If we prove that for some $t$, the above conditions cannot be simultaneously satisfied, then we are guaranteed that for at least one subset of $S$ of $B$,  we have
\begin{equation*}
	\forall_{S \subseteq B}\qquad \left(\bar{\valu}_i\left(S \cup \allocation_i\right)- \bar{\valu}_i\left(\allocation_i\right)\right) - C_\allocation(S) > 0.
\end{equation*}
This means that by taking back the items in $S$ from their owners and allocating them to agent $i$ we can increase the social welfare, which is in contradiction with the maximality of $Z'$. This in turn implies that a $t/2$-$\MMS$ allocation always exists. 
Based on this argument, our goal in this section is to find the largest value for $t$ such that satisfying all these conditions yields a contradiction. We denote this value by $t^*$. In the next two subsections, we prove two lower-bounds on $t^*$.
First, we show that $t^*\geq4/9$ which implies the existence of $2/9$-$\MMS$ allocation. 

\subsection{$t^* \geq 4/9.$}
Here we show that for $t=4/9$, Conditions $\mathsf{C_{1-4}}$ cannot be satisfied simultaneously. As a contradiction, let $B$ be a bundle that satisfies these conditions, and let $u_{i,i'}$ be the additive valuation function that defines $\valu_{i}(B)$. Let $\ite_1$ be the item in $B$ with the maximum contribution to $u_{i,i'}(B)$, that is, $\arg \max_{\ite \in B} \valu_i(\{\ite\}) $. Since by Condition $\mathsf{C_3}$, no pair of items have value at least $t/2$ to agent $i$, we know that the following holds:
$$
\forall_{b \in B \setminus \{b_1\}} \qquad u_{i,i'}(\{b\}) < t/4.
$$
Now, we proceed as follows: we consider an empty bag $\mathcal{B}$ and add item $\ite_1$ to the bag. Next, we add the rest of the items in $B$ to the bag one by one until the total value of the items in $\mathcal{B}$ for agent $i$ exceeds $t$. 

\begin{observation}\label{obs:bagfilling}
We have $\valu_{i}(\mathcal{B})<5t/4$. Therefore, $\valu_{i}(B \setminus \mathcal{B}) >1-5t/4$. 
\end{observation}
Observation \ref{obs:bagfilling} implies that we can divide the items in $B$ into two sub-bundles with value at least $\min(t,1-5t/4)$. 
Furthermore, by Condition $\mathsf{C_2}$ we know that the contribution of $B$ to $Z$ is less than $t$. Hence, the contribution of one of these two sub-bundles to $Z$ is less than $t/2$. 
Let $S$ be this sub-bundle. We have
\begin{align*}
		\left(\bar{\valu}_i\left(S \cup \allocation_i\right)- \bar{\valu}_i\left(\allocation_i\right)\right) - C_\allocation(S) &= \min(t, \min(t,1-5t/4)) - \bar{\valu}_i(\allocation_i) -  C_\allocation(S) \\
	&>  \min(t, 1-5t/4 ) - t/2 - C_\allocation(S) &\bar{\valu}_i(\allocation_i)<t/2\\
&>  4/9 - 2/9 - 2/9 &t=4/9\\
&=0.
\end{align*}
	This contradicts Condition $\mathsf{C_4}$. Therefore, a $2/9$-$\MMS$ allocation always exists. 
\begin{theorem}
	For any instance with fractionally subadditive valuations we can find a $2/9$-$\MMS$ allocation.
\end{theorem}
\subsection{$t^*>0.22962.$ \GS{$\times 2$}}
Here we improve the lower bound on $t^*$ via a more in-depth analysis. Note that, by Condition  $\mathsf{C_3}$ we know that the value of every pair of items to agent $i$ is at most $t/2$ . 
%This means that there is at most one item with value at least $t/2$ to agent $i$. 
Now, we consider two cases, either there exists an item with value at least $21t/64$, or all the items have value less than $21t/64$. We consider these two cases separately. 

\paragraph{Case 1.} If there exists an item with value at least $21t/64$, then we leverage the idea we used in the previous section. Let 
$b_1$ be the item with the largest value to agent $i$. By Condition $\mathsf{C_3}$, we know that the value of the rest of the items in $B$ is less than $11t/64$ to agent $i$. Via a similar argument as we made in the previous section, we can say that we can divide $B$ into two sub-bundles with value at least $\min(t,1-75t/64)$. Since by Condition $\mathsf{C_3}$ we know that the contribution of $B$ to $Z'$ is less than $t$, the contribution of one of these two sub-bundles to $Z'$ is less than $t/2$. Let $S$ be this sub-bundle. We have 
\begin{align*}
	\left(\bar{\valu}_i\left(S \cup \allocation_i\right)- \bar{\valu}_i\left(\allocation_i\right)\right) - C_\allocation(S) &= \min(t, \min(t,1-75t/64)) - \bar{\valu}_i(\allocation_i) -  C_\allocation(S) \\
	&>  \min(t, 1-75t/64 ) - t/2 - C_\allocation(S) &\bar{\valu}_i(\allocation_i)<t/2\\
	&>  1 - 75t/64 - t\\
	&= 1-139t/64.
\end{align*}
For $t\leq 64/139$, we have $1- 139t/64\geq 0 $ which implies $\left(\bar{\valu}_i\left(S \cup \allocation_i\right)- \bar{\valu}_i\left(\allocation_i\right)\right) - C_\allocation(S)>0$. This contradicts Condition $\mathcal C_4$. Therefore, for this case, we have the lower bound of $t^*> 64/139 \simeq 0.23021$.

\paragraph{Case 2.} For this case, we perform a more delicate analysis. Note that here we know that the value of each item to agent $i$ is less than $21t/64$. Assume that the items in $B$ are $b_1,b_2,\ldots,b_\ell$. Let $r_j$ be the value per contribution of item $\ite_j$, that is $r_j = \valu_i(\{\ite_j\})/ C_\allocation(\{\ite_j\})$, and suppose without loss of generality that the order of these items is according to their value per contribution, i.e.,
$
r_1 \geq r_2 \geq \ldots \geq r_\ell.
$ Furthermore, let $h$ be the smallest index, such that $\valu_i(\{\ite_1,\ite_2,\ldots,\ite_h\}) \geq t$, and let
\begin{align*}
\delta &= t/2 - C_\allocation(\{\ite_1,\ite_2,\ldots,\ite_{h-1}\})\\
\delta'&= t/2 - C_\allocation(\{\ite_{h+1},\ite_{h+2},\ldots,\ite_{\ell}\})\\
\gamma &= t-\valu_i(\{\ite_1,\ite_2,\ldots,\ite_{h-1}\})\\
\gamma' &= t-\valu_i(\{\ite_{h+1},\ite_{h+2},\ldots,\ite_{\ell}\})\\
\end{align*}

%For every $1 \leq j \leq \ell \leq k$ define $\delta_{j,\ell}$ as follows:
%$$
%\delta_{j,\ell} = \valu_i(\{\ite_j,\ite_{j+1},\ldots, \ite_\ell\}) - C_\allocation(\{\ite_j,\ite_{j+1},\ldots, \ite_\ell\}).
%$$
Then, we know that given that $\allocation$ maximizes social welfare, the following conditions hold.
\begin{enumerate}
	\item By Condition $\mathsf{C}_1$, we have $\valu_i(\{\ite_h\})\geq 1 - 2t +\gamma+\gamma'$. Therefore, since the value of the items is upper bounded by $11t/32$, we have $ 1 - 2t +\gamma+\gamma'<11t/32.$
	\item By Condition $\mathsf{C}_2$, the total contribution of the items in this bundle is less than $t$. Thus we have $C_\allocation(\{b_\ell\})<\delta + \delta'$. Also, we have $C_\allocation(\{b_\ell\}) \geq \max(\delta,\delta')$. \KM{The subscript should be $h$ instead of $\ell$.}
	 
	\item  By Condition$\mathsf{C}_2$, we have $0<\delta < \gamma$, otherwise taking back items $\{b_1,b_2,\ldots,b_{h-1}\}$ from other agents and allocating them to agent $i$ increases social welfare. With the same argument, we have $0<\delta'<\gamma'$.
	\item Since the items are sorted according to $r_i$, we have
	$$
	\frac{t - \gamma}{t/2-\delta} \geq r_h \geq \frac{t-\gamma'}{t/2-\gamma'}.
	$$  \KM{$\delta'$ instead of $\gamma'$ in the denominator.}
\end{enumerate}

Using standard mathematics \footnote{In fact, we used online tools for solving this constrained optimization problems.}, one can show that the smallest value $t$ that satisfies all the above constraints is grater than 
$$t = \frac{1}{42}(149-5\sqrt{673}) \simeq 0.459256.$$
 Indeed, for this case, for  $t=0.459256$, the allocation that maximizes social welfare, allocates each agent a bundle with value at least $t/2$. Therefore, a $0.22962$-$\MMS$ allocation always exists. 

Finally, combining these two cases implies that a $\min(0.234435,0.22962)$-$\MMS$ allocation always exists.
\begin{theorem}
	For any instance with fractionally subadditive valuations we can find a $0.22962$-$\MMS$ ($\simeq 20/87$-$\MMS$) allocation.
      \end{theorem}

      \subsection{On the Optimization Problem}

      I went back to the system in the paper by Masoud and his brother. I write $u_\ell$ and $c_\ell$ instead of $U_i^t(\{ b_\ell \})$ and similarly for $c$. 

      From $1 - 2t + \gamma + \gamma' \le u_\ell \le t/2$, we conclude $t \ge 2/5$. Here is a short argument that $t$ must be larger than $0.401$. If $u_\ell \le 198/1000$ (which is less than $0.2$) then
      $1 - 198/1000 \le 2t$ and hence $2t \ge 802/1000$ and hence $t \ge 0.401$.

      So we may assume $198/1000 \le t \le t/2$. If $\gamma + \gamma' \ge 5/2000$ then $2005/2000 \le 5t/2$ and hence $t \ge 401/1000$.

      So we may assume $\gamma + \gamma' \le 5/2000$. Then also $c_\ell \le \delta + \delta' \le 5/2000 = 1/400$. We must also have $(t - \gamma)/(t/2 - \delta) \ge u_\ell/c_\ell$. Since $u_\ell \ge 198/1000$ and $c_\ell \le 1/400$, the right hand side is at least $198 \cdot 400/1000 \approx 80$. However, the left hand side is approximately 2.

      


      \KM{Ignore everything below. It is not wrong, but I am not sure whether it leads anywhere.}

We want to find the minimum $t$ for which the following system of constrains is feasible. 
      We have the following constraints:
      \begin{enumerate}
\item $r_h = v_h/C_h$
\item $1 - 2t +\gamma+\gamma'<11t/32.$
\item $C_h \le \delta + \delta'$ and $C_h \ge \max(\delta,\delta')$.
  \item $0<\delta < \gamma$ and $0<\delta'<\gamma'$.
	\item 
	$\frac{t - \gamma}{t/2-\delta} \geq r_h \geq \frac{t-\gamma'}{t/2-\delta'}$ or equivalently  $C_h(t - \gamma) \ge v_h(t/2 - \delta)$ and $v_h(t/2 - \delta') \ge C_h(t - \gamma')$ or equivalently $(C_h - v_h/2)t \ge C_h\gamma - v_h \delta$. 
      \end{enumerate}
      In the paper by Masoud and his brother, there are the additional constraints $t > 0$ and $v_h \le t/2$ and $C_h \le t/2$.

      From the second constraint, we get $1 \le 75/32t$ and hence $t \ge 32/75 = 0.42666$.

      The variables are $v_h$, $C_h$, $t$, $\gamma$, $\gamma'$, $\delta$ and $\delta'$. For fixed values of $v_h$ and $C_h$, we obtain a linear program. The results of linear programs can be verified, see

      
    M. Dhiflaoui, S. Funke, C. Kwappik, K. Mehlhorn, M. Seel, E. Schömer, R. Schulte, and D. Weber.
    Certifying and Repairing Solutions to Large LPs, How Good are LP-solvers?.
    In SODA, pages 255–256, 2003.
    
    I have put a copy of the paper into our dropbox folder.

    I believe that the variables $\delta$ and $\gamma'$ can be eliminated.

    There are four inequalities involving $\delta$, namely $\delta \le C_h$, $\delta \le \gamma$ and $v_h \delta \ge C_h(t - \gamma) - v_ht/2$ and $\delta \ge C_h - \delta'$. If we have a solution to our system of constraints, then we may replace $\delta$ by $\min(C_h,\gamma)$. So we may delete the inequalities involving $\delta$, if we add the implied inequalities
    \begin{itemize}
    \item $v_hC_h \ge C_h(t - \gamma) - v_ht/2$  or $C_h \gamma \ge (C_h - v_h/2)t - v_hC_h$
    \item $v_h \gamma \ge C_h(t - \gamma) - v_ht/2$ or $(C_h + v_h)\gamma \ge (C_h - v_h/2)t$
    \item $C_h \ge C_h - \delta'$. This is always true.
    \item $\gamma \ge C_h - \delta'$ or $\delta' \ge C_h - \gamma$. 
    \end{itemize}
    This is actually a step of Fourier-Motzkin reduction: Solve all inequalities for one of the variables, say $x$. For any pair of inequalities $L \le x$ and $x \le R$, add the inequality $L \le R$. Then eliminate all inequalities involving $x$.

    Similarly, we may eliminate $\gamma'$. We have one upper bound on $\gamma'$ and two lower bounds. We eliminate all inequalities involving $\gamma'$ and add
    \begin{itemize}
    \item $1 + \gamma + \delta' \le 75t/32$
    \item $1 + \gamma + \frac{v_h(t/2 - \delta')}{C_h} \le 107 t/ 32$.
    \end{itemize}

    We still have variables, namely $v_h$, $C_h$, $t$, $\gamma$ and $\delta'$.

    For $\delta'$ we have the lower bounds $\delta' \ge 0$, $\delta' \ge C_h - \gamma$, and $1 + \gamma + \frac{v_h(t/2 - \delta')}{C_h} \le 107 t/ 32$ and the upper bounds $1 + \gamma + \delta' \le 75t/32$, $\delta' \le C_h$. We can elimate $\delta'$ at the cost of adding $6 = 3 \cdot 2$ inequalities. The new inequalities are:
    \begin{itemize}
    \item $1 + \gamma \le 75 t/32$.
    \item $C_h \ge 0$
    \item $1 + \gamma +C_h - \gamma \le 75t/32$ or $1 + C_h \le 75t/32$.
    \item $C_h - \gamma \le C_h$; this is always true.
    \item $(v_h + C_h)(1 + \gamma) + v_ht/2 \le (107 tC_h + 75 t v_h)/32$
    \item $C_h(1 + \gamma) + v_h(t/2 - C_h) \le 107 tC_h/ 32$ 
    \end{itemize}

    We still have variables $v_h$, $C_h$, $t$, and $\gamma$. I next try to eliminate $\gamma$. I am having three lower bounds $\gamma \ge 0$, $C_h \gamma \ge ....$, and $(C_h + v_h) \gamma \ge ...$ and three upper bounds $1 + \gamma \le 75t/32$, $C_h \gamma \le ....$, and $(v_h + C_h) \gamma \le ...$


==> src/extra.tex <==
	Before we end this section, we emphasize that for our setting, Lemma \ref{lem:fractorand} provides a stronger ex-post guarantee than Theorem \ref{thm:fei}: The ex-post guarantee of Lemma \ref{lem:fractorand} is $1/8$, while the ex-post guarantee of Theorem \ref{thm:fei} for our setting is $0$. \HA{Are we not done for this section then?} However, the analysis of Lemma \ref{lem:fractorand} is tailored to the assumption that $f_{i,j} \in \{0,1/2,1\}$.  
Alternatively, here we present Lemma \ref{lem:2}. This Lemma is similar to Theorem \ref{thm:1} with a tighter analysis of the value of each bundle ex-post. We defer the proof of Lemma \ref{lem:2} to the appendix. We also show in Lemma \ref{lem:3} that applying Lemma \ref{lem:2} to our setting yields $1/8$-$\MMS$ guarantee ex-post.

\begin{lemma} \label{lem:2}
	Assume that the valuations are additive. Let $\falloc$ be a fractional allocation and let $\items_{i}$ be the set of items that are strictly fractionally allocated to agent $i$. In addition, let $\falloc'$ be a partial allocation defined by variables $f'_{i,j}$ in the answer of the following linear program:
	\begin{align}
		\text{maximize }   &\sum_{1\leq i \leq n} \sum_{1 \leq j \leq m} f'_{i,j} \valu_{i}(\{\ite_j\})   \nonumber      \\
		\text{subject to } &   0 \leq f'_{i,j} \leq f_{i,j}& \forall {i,\ite_j \in \items_i}  \nonumber\\
		&   f'_{i,j}= 0 & \forall {i,\ite_j \notin \items_i}  \nonumber\\
		&  \sum_{1 \leq j \leq m} f'_{i,j} \leq 1 &\forall_i \label{opt:2}	
	\end{align}
	,and define $\beta_i$ as follows:
	$$
	\beta_i = \begin{cases}
		0 &\mbox{ if } \sum_j f'_{i,j}<1\\
		\min_{j: f'_{i,j} \neq 0}  \valu_i(\{\ite_j\})  &\mbox{ if } \sum_j f'_{i,j}=1
	\end{cases}
	$$ 
	Then there exists a randomized allocation 
	$\ralloc$ such that the ex-ante utility of agents  for $\ralloc$ is the same as the utility of agents in $\falloc$, and for every allocation $\allocation$ in the support of $\ralloc$ the following holds: 
	$$
	\forall_i \qquad  \valu_i(\allocation_i) \geq \valu_i(\ralloc) - \valu_i(\falloc') + \beta_i.
	$$	
\end{lemma}
\KM{Is this true? Consider the following example. We have one agent and three items of value 1, 1, and 0. The first two items are assigned with probability $1 - \epsilon$, the last item is assigned with probability $2\epsilon$. Then $v(\allocation) \ge 1$, since the agent is guaranteed one of the first two items. Also $v(\ralloc) = 2(1 - \epsilon)$. In $\falloc'$, the first item is assigned with probability $1 - \epsilon$ and the second with probability $\epsilon$. Thus $v(\falloc') = 1$. Finally $\beta = 1$. But
	$1 \ge 2(1 - \epsilon) - 1 + 1$ is wrong. I believe that you need to define $\beta$ as $v_i(b_j) f'_j$. The proof of Lemma 5.5 would still go through. }

Now, it only remains to bound $\valu_i(\falloc') - \beta_i$ from above for every agent $i$. In Theorem \ref{thm:1} we show that this value is bounded by $1/8$.

\begin{lemma}\label{lem:3}
	After Step (iii), for every agent $i$, we have $\valu_i(\falloc') - \beta_i \leq 1/8$. 
\end{lemma}
\begin{proof}
	Since for every item $\ite_{j}$ we have $f_{i,j} \in \{0,1,1/2\}$, the structure of $\falloc'$ is as follows: for every agent $i$ with $|\items_{i}| =1$, we have $\beta_i = 0$ and $\valu_i(\falloc') = f'_{i,j} \valu_{i}(\{\ite_j\})$, where $\ite_j$ is the only item in $\items_i$. Since  $\valu_{i}(\{\ite_j\}) \leq 1/4$ and $f'_{i,j} = 1/2$, we have $\valu_{i}(\falloc')-\beta_i \leq 1/8$. Furthermore, if  $|\items_{i}| >1$, 	assuming that $\ite_j,\ite_{j'}$ are the two most valuable items of $i$ in $\items_{i}$, we have $f'_{i,j} = f'_{i,j'} = 1/2$. Therefore, 
	\begin{align*}
		\valu_{i}(\falloc')-\beta_i 		&
		=
		\frac{\valu_{i}(\{\ite_j,\ite_{j'}\})}{2} - \valu_{i}(\{\ite_{j'}\})\\
		&	\leq 
		\frac{\valu_{i}(\{\ite_j\})+\valu_i(\{\ite_{j'}\})}{2}- \valu_{i}(\{\ite_{j'}\})\\ 
		&	\leq 
		\frac{\valu_{i}(\{\ite_j\})-\valu_i(\{\ite_{j'}\}))}{2} \\
		&	\leq 
		\frac{1}{8}.	  
	\end{align*} 
	
\end{proof}

==> src/omitted.tex <==
\section{Proof of Lemma \ref{lem:2}}
%
%{\color{blue} In this section, we prove Lemma~\ref{lem:2}. In \cite{babaioff2022best} it was shown how to convert a randomized allocation into a probability distribution over integral allocations. The construction is based on the Birkhoff---von Neumann theorem: Every fractional perfect matching can be written as a linear combination of integral perfect matchings. We adopt the construction to our setting and, in particular, exploit the fact that all $f_{ij}$ are half-integral.
%
%\begin{lemma} Assume that the valuations are additive and let $\falloc$ be a complete fractional allocation with $f_{ij} \in \{0, 1/2, 1\}$ for all $i$ and $j$. The there are two integral allocations $\allocation^1$ and $\allocation^2$ such that
%  \begin{itemize}
%  \item If $f_{ij} = 1$, $j$ is allocated to $i$ in both allocations, if $f_{ij} = 1/2$, $j$ is allocated to $i$ in one allocation, but not the other, and if $f_{ij} = 0$, $j$ is not allocated to $i$ in either allocation.
%  \item Let $\allocation$ be either of the two allocations. Then
%    \[ v_i(\allocation_i) \ge v_i(\ralloc) - \frac{\max \{ v_i(b_j)\, | \, f_{ij} = 1/2\}}{2} \]
%    for all $i$
%  \end{itemize}
%\end{lemma}
%\begin{proof}
%For each $i$, let $f_i = \sum_j f_{ij}$. Then $f_i$ is half-integral and the number of agents with non-integral $f_i$ is even, since $\sum_i f_i = \sum_{j} \sum_i f_{ij} = \sum_j 1 = m$. We pair the agents with non-integral $f_i$ arbitrarily, create a new dummy item for each pair, give the item value zero for all agents, and assign one-half of the dummy item to each agent in the pair. In this way all $f_i$ become integer.
%
%We now construct two allocations $\allocation^1$ and $\allocation^2$ such that $f_{ij}$ is equal to the fraction of allocations that assign $j$ to $i$. If $f_{ij} = 1$ we allocate $j$ to $i$ in both allocations, if $f_{ij} = 0$, we assign $j$ to $i$ in neither allocation, and if $f_{ij} = 1/2$ we assign $j$ to $i$ in exactly one of the two allocations. Care needs to be taken to be consistent accross agents. Construct a bipartite graph $G(X,Y)$ with parts $X$ and $Y$ as follows: For every item $j$ there is a vertex $y_j$ in $Y$ corresponding to item $\ite_j$. For every agent $i$, we have vertices vertices $x^i_1,x^i_2,\ldots,x^i_{t_i}$ to $X$, where $t_i$ is half the number of $j$ such that $f_{ij} = 1/2$.  We have the following edges. Consider a fixed $i$ and order the items $j$ with $f_{ij} = 1/2$ in decreasing order of value to $i$. Then $x^i_1$ is connected to the two most valuable items, $x^i_2$ is connected to the items whose values have ranks three and four, and so on. In this way each $x$- and each $y$-vertex has degree two and hence the graph decomposes into vertex disjoint cycles. Each cycle decomposes into two matchings and thus $G$ decomposes into two perfect matchings, say $M_1$ and $M_2$. We turn the matchings into allocations by indentifying, for each $i$, all vertices $x^i_*$. 
%
%Consider again a fixed agent $i$ and let $b_1$, $b_2$, \ldots, $b_{2t_i}$ be the items half-owned by $i$ in order of decreasing value for $i$. Then for all $\ell$, $1 \le \ell \le t_i$, $b_{2\ell - 1}$ and $b_{2\ell}$ are allocated to $i$ in different allocations. Hence the value of the $i$-th-bundle is either allocation $\allocation$ satisfies
%\[    v_i(\allocation_i) \ge v_i(b_2) + v_i(b_4) + \ldots + v_i(b_{2t_i})\]
%We can now bound $v_i(\falloc) - v_i(\allocation_i)$ from above. The $j$ with $f_{ij} \in \{0,1\}$ cancel out. For the $j$ with $f_{ij} = 1/2$ we obtain
%\begin{align*}
%  v_i(\falloc) - v_i(\allocation_i) &\le \frac{1}{2} \left(\sum_{1 \le \ell \le 2t_i} v_i(b_i) \right)  -  \sum_{1 \le \ell \le t_i} v_i(b_{2\ell}) \\
%                                    &= \frac{v_i(b_1)}{2} + \sum_{1 \le \ell < t_i} \left(\frac{v_i(b_{2\ell}) + v_i(b_{2\ell+1})}{2} - v_i(b_{2\ell})\right) + \frac{v_i(b_{2t_i})}{2} - v_i(b_{2t_i})\\
%  &\le  \frac{v_i(b_1)}{2}.
%\end{align*}
%\end{proof}
%
%
%
%
%}


In this section, we prove Lemma \ref{lem:2}. A major part of our proof is similar to the proof of Theorem \ref{thm:fei} in \cite{babaioff2022best}. The proof is based on Birkhoff -- von Neuman theorem which converts a fractional matching into an integral one. In a bipartite graph, a fractional perfect matching is an assignment of weights $w(e)$ to each edge $e$, such that $0 \leq w(e) \leq 1$, and the total sum of weights incident to each vertex is exactly equal to 1. We call a matching integral, if for every edge $e$, we have $w(e) \in \{0,1\}$. Birkhoff -- von Neuman theorem builds a connection between fractional and integral matchings.

\begin{theorem}[Birkhoff -- von Neuman]\label{bir}
	Every perfect fractional matching can be decomposed into a linear combination of integral perfect matchings.
\end{theorem}
Here, we use Theorem \ref{bir} as a black box. The idea is to convert a fractional allocation into a fractional allocation that can be represented by a perfect fractional matching and then use Theorem \ref{bir} to find a linear combination of integral allocations equivalent to the initial fractional allocation. Let $\falloc$ be a complete fractional allocation. First, we slightly modify allocation $\falloc$ as follows: for every agent $i$, define $f_i$ as $\sum_{1 \leq j \leq m} f_{i,j}$ and let 
$$
q = \sum_{1 \leq i \leq n} \lceil f_i \rceil - f_i.
$$
Note that since we assume that all the items are completely allocated in $\falloc$, $q$ is an integer. We add $q$ \emph{dummy} items $\ite_{m+1}, \ite_{m+2},\ldots,\ite_{m+q}$ with value 0 to all the agents to $\items$. 
For every agent $i$ and $m+1 \leq j \leq m+q$, we choose $f_{i,j}$ in a way that the resulting allocation is complete, and the total amount of items allocated to every agent $i$ is exactly equal to $\lceil f_i \rceil$.

We now construct a bipartite graph $G(X, Y)$ with parts $X$ and $Y$ as follows: for every item $1 \leq j \leq m+q$, there is a vertex $y_j$ in $Y$ corresponding to item $\ite_j$. Furthermore, for every agent $i$, we add $\lceil f_i \rceil$ vertices $x^i_1,x^i_2,\ldots,x^i_{\lceil f_i \rceil}$ to $X$. We determine the edges of $x^i_1,x^i_2,\ldots,x^i_{\lceil f_i \rceil}$ in a way that the following constraints are satisfied:
\begin{enumerate}
	\item \label{p1} Sum of the weights of the edges incident to every $x^i_\ell$ is exactly equal to 1.
	\item \label{p2} For every $\ell < \ell'$, vertices that are incident to $x^i_\ell$ are at least as valuable for agent $i$ as the vertices incident to $x^i_{\ell'}$.
	\item \label{p3} The total weight of the edges from vertices $x^i_1,x^i_2,\ldots,x^i_{\lceil f_i \rceil}$ to $y_j$ is exactly equal to $f_{i,j}$.
\end{enumerate}
Following classic graph notations, we denote the weight of edge $(x,y)$ in $G$ by $w(x,y)$ and denote the set of edges incident to vertex $x$ by $N(x)$. 
One can represent the above constraint in the following Program:
\begin{align*}
 	 (i)\qquad&   \sum_{y_j \in N(x^i_\ell)} w(y_j,x^i_\ell) = 1& \forall {1 \leq \ell \leq \lceil f_i \rceil} \\
 	(ii)\qquad & \valu_i(\{\ite_j\}) \geq \valu_i(\{\ite_{j'}\}) & \forall 1 \leq \ell \leq \ell' \leq 	\lceil f_i \rceil, y_j \in N(x^i_\ell), y_{j'} \in N(x^i_{\ell'})\\
 	(iii)\qquad &   \sum_{1 \leq \ell \leq \lceil f_i \rceil } w(y_j,x^i_\ell) = f_{i,j}& \forall {1 \leq j \leq m+q} 
\end{align*}
 By Property \ref{p3}, we have 
\begin{equation}\label{eq:valf}
	\valu_i(\falloc) = \sum_{1 \leq \ell \leq \lceil f_i \rceil} \sum_{y_j \in N(x^i_\ell)} \valu_i(\{\ite_j\}) w(y_j,x^i_\ell). 
\end{equation}
Furthermore, considering the definition of $\phi_i(\falloc)$ in Program \eqref{opt:2}, we have
\begin{equation}\label{def:phi}
	\phi_i(\falloc) = \sum_{y_j \in N(x^i_1)} w(x^i_1,y_j) \valu_i(\{\ite_j\}).
\end{equation}

Also, Note that by Property \ref{p1}, the weighted edges in $G$  constitute a perfect fractional matching. Hence, by Theorem \ref{bir}, we conclude that this fractional matching can be decomposed into a linear combination of integral perfect matchings. Let $M$ be one of these integral matchings. Since $M$ is perfect, every vertex $x^i_\ell$ in $G$ is incident to some edge $M(x^i_\ell)$. Now, consider the allocation $\allocation$ corresponding to $M$, that is, allocation that every agent $i$ receives items corresponding to vertices $M(x^i_1),M(x^i_2),\ldots, M(x^i_{\lceil f_i \rceil})$. We argue that in $\allocation$, value of agent $i$ for her share is at least $\valu_{i}(\falloc) - \phi_i(\falloc)$. 

For convenience, we assume without loss of generality that $M(x^i_\ell) = y_\ell$. Therefore, we have
\begin{align}
	\valu_i(\allocation_i) &= \sum_{1 \leq \ell \leq \lceil f_i \rceil}  \valu_i(\{\ite_\ell\})\label{eq:a1}
\end{align}
On the other hand, by Property \ref{p2}, for every $1 \leq \ell < \lceil f_i \rceil$ we have:
$$
\forall_{y_j \in N(x^i_{\ell+1})} \qquad \valu_i(\{\ite_j\}) \leq \valu_{i}(\{\ite_\ell\}).
$$ 
Therefore, by Property \ref{p1}, we have
\begin{equation}\label{ineq:a1}
	\sum_{y_j \in N(x^i_{\ell+1})}  \valu_i(\{\ite_j\}) w(y_j,x_{\ell+1}) \leq \valu_{i}(\{\ite_\ell\}).
\end{equation}
Combining Equation \eqref{eq:a1} with Inequality \eqref{ineq:a1} yields:
\begin{align}
	\valu_{i}(\allocation_i) &= \sum_{1 \leq \ell \leq \lceil f_i \rceil}  \valu_i(\{\ite_\ell\}) \nonumber\\
	&\geq \sum_{2 \leq \ell \leq\lceil f_i \rceil}	\sum_{y_j \in N(x^i_{\ell})}  \valu_i(\{\ite_j\}) w(y_j,x_{\ell}) \label{eq:aval} 
\end{align}
Therefore, considering Equation \eqref{def:phi} and Inequality \eqref{eq:aval} we have
\begin{align*}
	\valu_i(\falloc) - \valu_i(\allocation_i) &= 	\sum_{y_j \in N(x^i_{1})}  \valu_i(\{\ite_j\}) w(y_j,x_{1})\\
	&= \phi(\falloc).
\end{align*}


